EvGNN: An Event-driven Graph Neural Network Accelerator for Edge Vision

Edge vision systems combining sensing and embedded processing promise low-latency, decentralized, and energy-efficient solutions that forgo reliance on the cloud. As opposed to conventional frame-based vision sensors, event-based cameras deliver a microsecond-scale temporal resolution with sparse information encoding, thereby outlining new opportunities for edge vision systems. However, mainstream algorithms for frame-based vision, which mostly rely on convolutional neural networks (CNNs), can hardly exploit the advantages of event-based vision as they are typically optimized for dense matrix-vector multiplications. While event-driven graph neural networks (GNNs) have recently emerged as a promising solution for sparse event-based vision, their irregular structure is a challenge that currently hinders the design of efficient hardware accelerators. In this paper, we propose EvGNN, the first event-driven GNN accelerator for low-footprint, ultra-low-latency, and high-accuracy edge vision with event-based cameras. It relies on three central ideas: (i) directed dynamic graphs exploiting single-hop nodes with edge-free storage, (ii) event queues for the efficient identification of local neighbors within a spatiotemporally decoupled search range, and (iii) a novel layer-parallel processing scheme allowing for a low-latency execution of multi-layer GNNs. We deployed EvGNN on a Xilinx KV260 Ultrascale+ MPSoC platform and benchmarked it on the N-CARS dataset for car recognition, demonstrating a classification accuracy of 87.8% and an average latency per event of 16$\mu$s, thereby enabling real-time, microsecond-resolution event-based vision at the edge.

==> hw/matvec_eq.tex <==
\begin{equation} 
\label{eq:matvec}
\begin{split}
    &\mathbf{message} = W_{C_{out} \times C_{in}} \cdot \mathbf{x}_{C_{in}\times 1} \\
    &=  \begin{bmatrix}
            w_{1,1}&       \cdots & w_{1,C_{in}}      \\
            \vdots&        \ddots & \vdots            \\
            w_{C_{out},1}& \cdots & w_{C_{out},C_{in}}
    \end{bmatrix}
    \begin{bmatrix}
             x_1       \\
             \vdots    \\
             x_{C_{in}}
    \end{bmatrix} \\
    &= \sum_{j=1}^{C_{in}} x_j
    \begin{bmatrix}
              w_{1,j}      \\
              \cdots             \\
              w_{C_{out},j}
    \end{bmatrix}
    = \begin{bmatrix}
          \sum x_j \cdot w_{1,j}      \\
                   \cdots             \\
          \sum x_j \cdot w_{C_{out},j}
      \end{bmatrix}
\end{split}
\end{equation}

